MARS: Malleable Actor-Critic Reinforcement Learning Scheduler

In this paper, we introduce MARS, a new scheduling system for HPC-cloud infrastructures based on a cost-aware, flexible reinforcement learning approach, which serves as an intermediate layer for next generation HPC-cloud resource manager. MARS ensembles the pre-trained models from heuristic workloads and decides on the most cost-effective strategy for optimization. A whole workflow application would be split into several optimizable dependent sub-tasks, then based on the pre-defined resource management plan, a reward will be generated after executing a scheduled task. Lastly, MARS updates the Deep Neural Network (DNN) model based on the reward. MARS is designed to optimize the existing models through reinforcement mechanisms. MARS adapts to the dynamics of workflow applications, selects the most cost-effective scheduling solution among pre-built scheduling strategies (backfilling, SJF, etc.) and self-learning deep neural network model at run-time. We evaluate MARS with different real-world workflow traces. MARS can achieve 5%-60% increased performance compared to the state-of-the-art approaches.

==> future.tex <==
\section{Future Work}
\label{future_work}
In our future work, we are considering to implement a user friendly protocol to communicate with HPC resource manager, and save multiple models from same training sets. We also need to address the issue that reward value can be different between HPC systems, considering a mean value between multiple systems. 

Next, our proposal can be expanded to support could infrastructure where the resources are unlimited but the cost value is high, using same principle we can expand \texttt{MARS} to support Docker \cite{Docker}, Kubernetes \cite{Kubernetes}, and other container based solutions. 


